Novel View Video Prediction Using a Dual Representation

We address the problem of novel view video prediction; given a set of input video clips from a single/multiple views, our network is able to predict the video from a novel view. The proposed approach does not require any priors and is able to predict the video from wider angular distances, upto 45 degree, as compared to the recent studies predicting small variations in viewpoint. Moreover, our method relies only onRGB frames to learn a dual representation which is used to generate the video from a novel viewpoint. The dual representation encompasses a view-dependent and a global representation which incorporates complementary details to enable novel view video prediction. We demonstrate the effectiveness of our framework on two real world datasets: NTU-RGB+D and CMU Panoptic. A comparison with the State-of-the-art novel view video prediction methods shows an improvement of 26.1% in SSIM, 13.6% in PSNR, and 60% inFVD scores without using explicit priors from target views.

==> supple.tex <==
% % Template for ICIP-2018 paper; to be used with:
% %          spconf.sty  - ICASSP/ICIP LaTeX style file, and
% %          IEEEbib.bst - IEEE bibliography style file.
% % --------------------------------------------------------------------------
% \documentclass{article}
% \usepackage{spconf,amsmath,graphicx}

% \usepackage{times}
% \usepackage{epsfig}
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}

% \usepackage{cuted}
% \usepackage{capt-of}

% \usepackage{color}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}

% % \AtBeginDocument{\setlength{\FullWidth}{\textwidth}}


% % Example definitions.
% % --------------------
% \def\x{{\mathbf x}}
% \def\L{{\cal L}}

% % Title.
% % ------


\title{Novel View Video Prediction Using a Dual Representation \\ Supplementary Material}

\name{Sarah Shiraz, Krishna Regmi, Shruti Vyas, Yogesh S. Rawat, Mubarak Shah
}
\address{Center for Research in Computer Vision (CRCV)-University of Central Florida}

% \begin{document}


%\ninept
%
% %%%%%{-35pt}

\maketitle

% \section{Network Details}
% Include more details about view dependent network $V_T$ \SV{Do you mean the diagram explaining both global and view dependent rep?}
% \SV{You can include your network details for all parts of the network here. Use either a figure or a table format to show details e.g. conv2D, kernel size, batch norm, concat etc.}
\section{Additional Network Details}

 \begin{figure*}[t]
 \begin{center}
    \includegraphics[width=.99\textwidth]{images/WACVPanoptic72Views-1.pdf}
    \end{center}
\caption{Qualitative results on CMU Panoptic dataset for 72 views experiment with five input views showing three different samples. The resolution is $56 \times 56$.
% (300%%% zoom-in for better visualization.) %[[maybe we need to remove few images from the figure]]
}
\label{fig:Panoptic72Views}
\end{figure*}

\begin{figure}[t]
\begin{center}
  %%%%%{-5pt}

\includegraphics[width=.47\textwidth, height=3cm]{images/CVPRPlot.pdf}
\end{center}
  %%%%%{-10pt}

  \caption{SSIM and PSNR scores vs the number of input views. Higher number of views help better prediction quality. The plots show scores for 5 randomly chosen query views.
%   \YSR{the text reads funny, you may want to fix this...}
  }
\label{fig:effectNumViews}
% \label{fig:onecol}
  %%%%%{-10pt}
\end{figure}


\textit{Video encoder} is a modified I3D network\cite{carreira2017quo} where the modifications are: (i) remove max pooling layer after block 2, (ii) for max pooling in block 3 \& 4, stride is set to 2$\times$1$\times$1, (iii) Add 1$\times$1$\times$1 convolutional layer before average pooling, to reduce the number of feature maps to 256. 
Finally, $V_E$ is initialized with I3D weights pre-trained on ImageNet\cite{denglarge}.
% The maxpool layer after block 2 is removed. For maxpool layers in block 3 and 4, we use  the stride of  2 $\times$ 1 $\times$ 1. Also, we add a 1 $\times$ 1 $\times$ 1 convolutional layer before the AvgPool operation and extract the encoder features.
% This reduces the number of feature maps to 256. The  encoder is initialized with I3D weights pre-trained on ImageNet \cite{denglarge}.
% I3D parameters, while the last convolutional layer is randomly initialized. 

\textit{View Embedder, VE} is a trilinear interpolation layer which takes the view information ($v_i$ or $v_q$) of size (1$\times$1$\times d$), where, $d$ is the number of view dimensions.and interpolates the spatial size to match with that of the encoder features in case of the View Dependent Block and the Global Representation Block ( i.e. $v_i$ and $v_i - v_q$) and convLSTM features in the case of Video Decoder ($v_q$) respectively, as we can see from the Network Diagram in the manuscript.

\textit{View Dependent Block, $V_{T}$} consists of two fully-connected layers of size $d^p \times d^p$ and $2d^p \times d^p$ where $d^p$ is the number of view dimensions in $v_{i}^{p} $ or $ v_{q}^{p}$.
Next, it uses a bidirectional convLSTM with 64 3 $\times$ 3 $\times$ 3 kernels; followed by a unidirectional convLSTM with 128 3 $\times$ 3 $\times$ 3 filters in the convolutions.
The output features from the Video Encoder, $e_{i}^{'}$ and the relative view embeddings from the View Embedder are concatenated channelwise and passed as input to this block. 

\textit{Global Representation Block} 
% Similar to View Dependent Block, this block
also consists of a bidirectional convLSTM followed by a unidirectional convLSTM. Here, the first convLSTM consists of 128 3 $\times$ 3$ \times$ 3 filters whereas the second one uses 256 3 $\times$ 3$\times$ 3 filters.

\textit{Query Network}
% It 
is a single-layer convolutional network with 256 filters and filter size of 5 $\times$ 5 $\times$ 5.

\textit{Video Decoder}
has 8 convolutional layers (combined with upsampling layers) with kernel sizes 5$\times$ 5 $\times$ 5 and 256, 256, 256, 256, 256, 128, 64, 3 filters respectively. The second last layer uses kernel size 3 $\times$ 3 $\times$ 3. The final layer is the Tanh activation.


\textit{Discriminator}
% The discriminator 
is a 6-layered 3D CNN with 3 $\times$ 3$\times$ 3 kernels and strides of 2 $\times$ 2 $\times$ 2. The number of filters in each layer is [16, 32, 64, 128, 256, 256] respectively. After the last convolution, we add a fully connected layer followed by Sigmoid activation.

\section{Additional Results}

% \subsection{Videos}
% The videos for our results can be found in the attached file videos.zip. It contains six videos showing results for CMU Panoptic \cite{joo2015panoptic} Large-scale Multiview Experiment (56 $\times$ 56), comparison with the state-of-the-art \cite{lakhal2019view} (56 $\times$ 56), View Interpolation experiment, additional results on 224 $\times$ 224 resolution, NTU-RGB+D dataset \cite{shahroudy2016ntu} multi-input view setup (56 $\times$ 56) and comparison with the state-of-the-art (112 $\times$ 112). For the view interpolation experiment, we perform feature space view interpolation between the discrete views provided in the dataset and show smooth transition between different viewpoints for an action.
% The video file names correspond to the experimental setup.


% It can be observed that the proposed method is able to successfully generate good quality videos from a novel view and also preserves human motion and color information. As compared with the video based baseline view-lstm \cite{lakhal2019view}, it produces much sharper frames. The view interpolation results are shown for the query views in between the actual viewpoints provided by the dataset. These viewpoints are not present in the dataset and we show the ground truth only for the viewpoints present in the dataset. It can be seen that the results are equally good for such viewpoints which reveals the consistency of the 3D representation learned by the proposed network.

% \clearpage


% ------------ FIGURE 72views START ---------------- %




\begin{table*}[t]
 \small
  \centering
  \renewcommand{\tabcolsep}{2mm}  
  
  \caption{\small Quantitative results (SSIM, PSNR and FVD scores) for 72 views experiment on CMU Panoptic dataset on $56 \times 56$ resolution. For each panel, input views are fixed to ($v_1$,$v_2$,$v_3$,$v_4$,$v_5$) and we test output views from $v_6$ to $v_{24}$. 
  }

  \label{tab:72ViewsSSIMResultsTry}
    \begin{tabular}
    {|l|c c c|c c c|c c c|c c c|}

                \cline{1-10}

        \textbf{Query} & \multicolumn{3}{c|} {\textbf{Panel 4}}  & \multicolumn{3}{c|} {\textbf{Panel 5}}& \multicolumn{3}{c|} {\textbf{Panel 17}}
        \\

        \cline{2-10}
        % \hline
        
         \textbf{View}&\textbf{SSIM($\uparrow$)}&  \textbf{PSNR($\uparrow$)} & \textbf{FVD($\downarrow$)}&\textbf{SSIM($\uparrow$)}&\textbf{PSNR($\uparrow$)} &\textbf{FVD($\downarrow$)}&\textbf{SSIM($\uparrow$)}& \textbf{PSNR($\uparrow$)} & \textbf{FVD($\downarrow$)}\\
                % \cline{1-10}

        \hline
        \hline
        
        \textbf{$v_6$ } &0.814&  24.46 & 7.58&0.852&26.79 &11.79&0.855& 25.94 & 11.80  \\
        \textbf{$v_7$ } &0.795&  24.56 & 11.64&0.843&25.66 &13.17&0.820& 26.06 & 13.17 \\
        \textbf{$v_8$ } &0.794&  24.02 & 10.49&0.842&25.94 &16.01&0.834& 26.15 & 16.04 \\
        \textbf{$v_9$ } &0.813&  24.7 & 10.66&0.827&25.16 &17.65&0.795& 25.18 & 14.23 \\
        \textbf{$v_{10}$ } &0.829&  25.58 & 10.91&0.828&24.99 &14.80&0.807& 25.69 & 14.82 \\
        
        \textbf{$v_{11}$ } &0.836&  25.36 & 11.98&0.823&24.21 &12.72&0.809& 24.33 & 12.67 \\
        \textbf{$v_{12}$ } &0.871&  26.50 & 8.24&0.807&23.17 &10.92&0.784& 24.17 & 10.89 \\
        \textbf{$v_{13}$ } &0.834&  25.09 & 10.80&0.832&23.61 &13.33&0.805& 24.62 & 13.32 \\
        \textbf{$v_{14}$ } &0.811&  24.17 & 15.01&0.808&23.26 &11.86&0.789& 24.25 & 11.85 \\
        \textbf{$v_{15}$ } &0.827&  24.7 & 8.24&0.844&24.43 &16.60&0.797& 23.90 & 16.60 \\
        \textbf{$v_{16}$ } &0.852&  26.48 & 12.69&0.860&25.06 &10.84&0.813& 24.62 & 10.87 \\
        \textbf{$v_{17}$ } &0.868&  26.80 & 11.01&0.835&23.76 &10.50&0.808&24.31 & 10.48 \\
        \textbf{$v_{18}$ } &0.846&  27.43 & 10.44&0.817&24.82 &9.86&0.810& 24.14 & 9.84 \\
        \textbf{$v_{19}$ } &0.829&  25.01 & 12.25&0.836&23.90 &13.71&0.816& 24.60 & 13.70 \\
        \textbf{$v_{20}$ } &0.820&  25.02 & 13.26&0.851&25.68 &13.97&0.827& 24.95 & 13.97 \\
        \textbf{$v_{21}$ } &0.822&  25.06 & 12.14&0.811&24.60 &14.91&0.832& 25.83 & 14.89 \\
        \textbf{$v_{22}$ } &0.810&  24.82 & 10.08&0.839&24.44 &15.04&0.804& 24.65 & 15.04 \\
        \textbf{$v_{23}$ } &0.824&  25.15 & 15.53&0.839&24.73 &14.05&0.811& 24.66 & 14.02 \\
        \textbf{$v_{24}$ } &0.835&  25.61 & 15.94&0.823&23.65 &13.31&0.750& 20.59 & 14.70 \\
                % \cline{1-10}
                \hline
                % \hline
        % \textbf{Average} &0.827&  25.25 & 11.52&0.832&24.62 &13.42&0.808& 24.66 & 13.31  \\
        
        
        
        % \cline{1-10}
        %   \hline

    \end{tabular}
\end{table*}


\begin{figure*}[t]
% \begin{figure}[htbp]
\begin{center}
%   \includegraphics[width=0.81\linewidth]{images/72ViewsDemo1.pdf}
\includegraphics[width=0.78\linewidth]{images/WACV72ViewsDemo.pdf}
%   %%%%%{-10pt}
\end{center}
   \caption{\small  Qualitative Results on CMU Panoptic dataset showing synthesized frames employing  five input views (v$_1$ through v$_5$) and randomly selected query  views from the remaining views ($v_6$ - $v_{24}$) for each panel. 
%   The \MS{query}  views for each panel are as follows:  \textbf{Panel 4}: $v_6,$ $v_7,$ $v_{8,}$ $v_{13},$ $v_{15},$$v_{16},$ $v_{17},$ $v_{18},$ $v_{20}$,$v_{22},$ $v_{24},$  \textbf{Panel 5}: $v_8,$ $v_9,$ $v_{11},$ $v_{13},$ $v_{15},$ $v_{16},$ $v_{17},$ $v_{18},$ $v_{19},$ $v_{23},$ $v_{24}$. \textbf{Panel 17:} $v_{12},$ $v_{14},$ $v_{15},$ $v_{23},$ $v_{22}$,$v_{18},$ $v_{16},$ $v_{17},$ $v_{21},$ $v_{7},$ $v_{13}$.
    We show 3 samples and the resolution is $56 \times 56$. }
\label{fig:panoptic_72Views_panel4}
% %%%%%{-15pt}
\end{figure*}



\subsection{CMU Panoptic Dataset \cite{joo2015panoptic}}


\noindent \textbf{Large-scale Multiview Experiment. }
We provide additional qualitative results on CMU Panoptic Dataset. 
% To further validate the applicability of our method, we move to higher number of views for the second experiment and select 72 views from CMU Panoptic Dataset. Specifically, we select 3 panels (panel number 4, 5 and 17 ) and use all (24) views from each panel, totalling 72 views (3 panels with 24 viewpoints per panel).  We  use  56  viewpoints  for  training,  and  16  viewpoints  for the testing. We use a split of 6,244 training and 1,132 test samples,  however here each sample contains 72 video clips from each view. Training on this many number of views was a significant  challenge for us as it introduced  a lot of randomness in the input and output views. Adversarial loss and perceptual loss helped in handling the blur of the generated output clips. While training, for a randomly selected panel, we randomly select 5 input views and generate a novel view from the same panel. 
% % The batch size used was 8. 



Figure \ref{fig:Panoptic72Views} depicts the frames at time t = 0, 8 and 15 for five input views as well as the synthesized frames and the corresponding ground truth frames from the query view.
 
The detailed quantitative evaluation is provided in Table \ref{tab:72ViewsSSIMResultsTry}. The evaluation is conducted per panel separately. For each panel, the  viewpoints from $v_1$ to $v_5$ are fixed as input views and the output video clips for the remaining 19 viewpoints ($v_6$ to $v_{24}$) are synthesized. 
% So input views points are ($v^1$,$v^2$,$v^3$,$v^4$,$v^5$) and we test on output view points from $v^6$ to $v^{24}$.  
The SSIM, PSNR and FVD scores are provided in Table \ref{tab:72ViewsSSIMResultsTry}. The average scores for panel 4, 5 and 17 are 

For the same configuration, we provide additional qualitative results in Figure \ref{fig:panoptic_72Views_panel4} for randomly selected query views from the pool of viewpoints from $v_6$ to $v_{24}$. It can be observed that video frames and motion are equally good for each of the query views given the five input views as shown.




\begin{table*}[]
 \small
  \centering
  \renewcommand{\tabcolsep}{3mm}  
  
  \caption{\small SSIM and PSNR scores for investigating the effect of varying the number of input views. We randomly select 9 query views $v_k$ from panel 4 and increase the input views from 1 to 5.}
%   %%%%%{5pt}
  \label{tab:multiple_views_effect}
    \begin{tabular}{|l|c|c|c|c|c|c|}
    \hline
         & \multicolumn{1}{c|} {\textbf{Query View}}  & \multicolumn{5}{c|} {\textbf{Input Views}}\\
         \cline{2-7}
       \textbf{Metrics}  &
        \textbf{$v_k$} &  \textbf{$(v_1)$} & \textbf{($v_1 ,v_2$)}  & \textbf{($v_1, v_2, v_3$)}  & \textbf{($v_1, v_2, v_3, v_4$)} & \textbf{($v_1, v_2, v_3, v_4, v_5$)}  
        \\
        % \midrule
        % \midrule
        \hline
        \hline
        & \textbf{$v_6$}  & 0.789 & 0.803 & 0.808 &0.812&0.814 \\
        &  \textbf{$v_{10}$}  & 0.806 & 0.818 & 0.820 & 0.822 &0.829  \\
       &  \textbf{$v_{11}$}  & 0.796 & 0.815 & 0.823 & 0.824 &0.836  \\
        & \textbf{$v_{12}$}  & 0.858 & 0.867 & 0.870 &0.871&0.871 \\
       \textbf{SSIM($\uparrow$)}  & \textbf{$v_{13}$}  & 0.807 & 0.816 & 0.820 &0.819&0.834 \\
        & \textbf{$v_{14}$}  & 0.776 & 0.781 & 0.784 &0.784&0.811 \\
        & \textbf{$v_{16}$}  & 0.841 & 0.844 & 0.847 &0.850&0.852 \\
        & \textbf{$v_{17}$}  & 0.846 & 0.856 & 0.857 &0.858&0.868\\
       & \textbf{$v_{20}$}  & 0.786 & 0.797 & 0.809 &0.812&0.820 \\
    
        % \cline{2-7}
        % & \textbf{Average}  & \textbf{0.811} & \textbf{0.821} & \textbf{0.826} &\textbf{0.828}&\textbf{0.835} \\
        
       
        
        
        % \hline
        % & \textbf{Average}  & 0.816 & 0.867 & 0.870 &0.871&0.871 \\
        
        \hline
        & \textbf{$v_6$}  & 23.51 & 24.06 & 24.27 &24.41&24.46 \\
         &  \textbf{$v_{10}$}  & 24.48 & 24.87 & 25.00 &25.02&25.58 \\
          &  \textbf{$v_{11}$}  & 24.17 & 24.92 & 25.28 &25.30&25.36 \\
        & \textbf{$v_{12}$}  &25.60& 26.14 & 26.35 & 26.46 &26.50 \\
        \textbf{PSNR($\uparrow$)} & \textbf{$v_{13}$}  & 24.82 & 25.16 & 25.25 &25.22&25.09 \\
         & \textbf{$v_{14}$}  &23.34& 23.54 & 23.63 & 23.80 &24.17 \\
         & \textbf{$v_{16}$}  & 25.98 & 26.14 & 26.32 &26.40&26.48 \\
        
        & \textbf{$v_{17}$}  & 25.90 & 26.56 & 26.73 &26.80&26.80 \\
        & \textbf{$v_{20}$}  & 23.99 & 24.29 & 24.64 &24.83&25.02 \\
        % \cline{2-7}
        % & \textbf{Average}  & \textbf{24.64} & \textbf{25.06} & \textbf{25.27} &\textbf{25.36}&\textbf{25.42} \\
        
     \hline

    \end{tabular}
\end{table*}


% %%%%%{10pt}


\begin{table*}
 \small
  \centering
  \renewcommand{\tabcolsep}{3mm}  
  
  \caption{\small Quantitative comparison with state-of-the-art viewLSTM\cite{lakhal2019view} on CMU Panoptic dataset at $56 \times 56$ resolution and single-input setup. Our method performs significantly better than SOTA viewLSTM\cite{lakhal2019view} on all three evaluation metrics for all input-output view combinations. 
%   \MS{try to move this table up; there is lot of empty space; reviewers may not see these tables}
  }  

  
%   %%%%%{5pt}
  \label{tab:comparison_with_vLSTM_Panoptic_3Views}
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        % \toprule
        \hline
        \textbf{} & & \multicolumn{6}{c|} {\textbf{Input View $\xrightarrow{}$ Output View}} & \textbf{Average}
        \\
        % \cline{3-4}
        % \textbf{}& & \hspace{3.9mm} \textbf{{SSIM}}  \textbf{($\uparrow$)}  \hspace{3.9mm} & \hspace{3.9mm} \textbf{{PSNR}} \textbf{($\uparrow$)}   \hspace{3.9mm} & \hspace{3.9mm} \textbf{{FVD}} \textbf{($\downarrow$)} \hspace{3.9mm}  \\
        \cline{3-8}

        \textbf{Method}& \textbf{Metrics} &  \textbf{{$v_1$ $\xrightarrow{}$ $v_2$}} & \textbf{{$v_1$ $\xrightarrow{}$ $v_3$}} & \textbf{{$v_2$ $\xrightarrow{}$ $v_1$}} & \textbf{{$v_2$ $\xrightarrow{}$ $v_3$}} & \textbf{{$v_3$ $\xrightarrow{}$ $v_1$}} &\textbf{{$v_3$ $\xrightarrow{}$ $v_2$}} & \textbf{Score} \\
        % \cite{lakhal2019view} \hspace{4mm}  \textbf{Ours} & \cite{lakhal2019view} \hspace{4mm} \textbf{Ours}  
        \hline
        \hline
        
        & \textbf{{SSIM}}  \textbf{($\uparrow$)}  & 0.675 & 0.684 &0.686 & 0.673 & 0.690 & 0.680 & 0.681\\
      \cite{lakhal2019view} &\textbf{{PSNR}}  \textbf{($\uparrow$)} & 23.03 & 23.16 & 22.56 & 23.07 & 22.69 & 23.24 & 22.96  \\
        & \textbf{{FVD}}  \textbf{($\downarrow$)} & 22.43  &  25.67 & 20.62 & 25.73 & 20.32 & 22.48 & 22.87 \\

                \hline
                
        & \textbf{{SSIM}}  \textbf{($\uparrow$)}  & 0.740 & 0.751 &0.753 & 0.748 & 0.742 & 0.732 & 0.744\\
      \cite{Wiles_2020_CVPR} &\textbf{{PSNR}}  \textbf{($\uparrow$)} & 21.33 & 21.75 & 22.53 & 21.41 & 21.44 & 20.70 & 21.53  \\
        & \textbf{{FVD}}  \textbf{($\downarrow$)} & 18.23  &  18.98 & 16.23 & 17.95 & 17.88 & 16.42 & 17.62 \\

                \hline

        & \textbf{{SSIM}}  \textbf{($\uparrow$)}  & 0.862 &  0.853 & 0.852 & 0.861 & 0.858 & 0.876 & \textbf{0.859}\\
        \textbf{Ours} &\textbf{{PSNR}}  \textbf{($\uparrow$)}  & 26.37 &  25.48 & 25.85 & 25.58 & 26.34 & 26.87 & \textbf{26.08}\\
        & \textbf{{FVD}}  \textbf{($\downarrow$)} & 8.51 & 10.12 & 9.21 & 9.98  & 8.93 & 8.20  & \textbf{9.15} \\
        
        
            \hline

    \end{tabular}
    % %%%%%{-10pt}
\end{table*}



% %%%%%{12pt}
% %%%%%{10pt}



\noindent \textbf{Effect of Multiple Input Views. }

% To examine the effect of number of input views on video quality, we perform multiple experiments by increasing the number of input views from one to five and report the results in Figure \ref{fig:effectNumViews}. As expected, with an increase in the number of input views the video quality improves. This validates that the network is able to capture and aggregate the features pertinent to each view and exploit them to synthesize the query view.






This analysis is conducted to understand the impact of multiple input views on the quality of the synthesized videos. 
The number of input clips is increased from 1 to 5 to synthesize the video from the query view and report the results in Figure \ref{fig:effectNumViews}. As expected, with an increase in the number of input views the video quality improves. This validates that the network is able to capture and aggregate the features pertinent to each view and exploit them to synthesize the query view.

The SSIM and PSNR scores are reported for the synthesized video frames in Table \ref{tab:multiple_views_effect}. The input and query views are selected from Panel 4 for this analysis. We observe that the scores improve as the number of input view increases from single to multiple views. This is possible since the multiple input views are successful at providing greater scene details useful to learn to synthesize the query view.


% To investigate the effect of using multiple input views, we perform testing by increasing number of input views. We pick panel 4 for our testing and test randomly selected output views by increasing number of input views from 1 to 5. The quantitative results in terms of SSIM and PSNR are given in Table \ref{tab:multiple_views_effect}. The scores increase as we move from single to multiple input views, as can be observed from the table.

\noindent \textbf{Higher Resolution Experiment}
For the same setup, we also conduct experiment on 224 $\times$ 224 resolution. The qualitative results are shown in Figure \ref{fig:panoptic_3views_224x224}. The model is able to preserve fine details and produce sharper frames with an SSIM and PSNR score of 0.812 and 24.55, respectively.


% %%%%%{12pt}

\begin{figure*}[t]
% \begin{figure}[htbp]
\begin{center}
%   \includegraphics[width=0.99\linewidth]{images/Results-Pan-3Views-Comparison-Half.pdf}

% \includegraphics[width=0.7\linewidth]{images/Panoptic224x224-New1.pdf}
\includegraphics[width=0.92\linewidth]{images/Panoptic224x224-Final.pdf}
  %%%%%{-10pt}
\end{center}
   \caption{\small Qualitative Results on CMU Panoptic dataset with multi-view input
%   $v^{i} $ $\xrightarrow{}$ $v^j$ 
   setup. We show three samples and the resolution is $224 \times 224.$ 
%   \SV{show more frames, not just 3, you have space.}
% \YSR{add more frame to each video sample here as well... not just 3...}
   }
\label{fig:panoptic_3views_224x224}
% %%%%%{-10pt}
\end{figure*}

\noindent \textbf{Comparison with viewLSTM\cite{lakhal2019view}. }
Here, we provide additional qualitative and quantitative evaluation of our proposed approach with state-of-the-art  viewLSTM \cite{lakhal2019view} in Figure \ref{fig:panoptic_3views_comparison1} and Table \ref{tab:comparison_with_vLSTM_Panoptic_3Views} respectively. The experimental details are provided in the manuscript in Section 5.1.

%The qualitative results for the comparison of the proposed method with the state-of-the-art viewLSTM \cite{lakhal2019view} is provided in Figure \ref{fig:panoptic_3views_comparison1}. 
In Figure  \ref{fig:panoptic_3views_comparison1}, we show three samples from different input viewpoints, each at three time instances, t = 0, 8 and 15. The actors in the images are performing different actions. Qualitatively, our proposed method is successful at synthesizing better images with sharper foreground-background boundaries and also capture the motion of the person along the temporal sequence.

The detailed quantitative result in Table \ref{tab:comparison_with_vLSTM_Panoptic_3Views} provides the performance of our method and the state-of-the-art  viewLSTM \cite{lakhal2019view} for view transformation between the Panels 2,4 and 10 (Node 10). The SOTA method uses the query view skeleton priors to synthesize the query RGB frames, whereas our method doesn't utilize the skeleton information from the query view. We observe that our proposed method outperforms the existing SOTA by huge margins for all evaluation metrics. 



\begin{figure*}[t]
% \begin{figure}[htbp]
\begin{center}
%   \includegraphics[width=1.0\linewidth]{images/WACVResults-Pan-3Views-ComparisonFFF.pdf}
   \includegraphics[width=0.9\linewidth]{images/WACVResults-Pan-3Views.pdf}
%   %%%%%{-10pt}
\end{center}
   \caption{\small Qualitative Results showing the comparison of our proposed method with state-of-the-art method viewLSTM \cite{lakhal2019view} on CMU Panoptic dataset. We show 3 samples, each with frames at time t =0, 8 and 15; and the resolution is $56 \times 56$.}
\label{fig:panoptic_3views_comparison1}
% %%%%%{-15pt}
\end{figure*}


% \begin{figure*}[t]
% \begin{center}
% % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%   %\includegraphics[width=0.8\linewidth]{egfigure.eps}
%   \includegraphics[width=.90\textwidth]{images/WACVNetworkAblation-Fig1.pdf}
%   %%%%%{-10pt}
% \end{center}
%   \caption{Qualitative results showing Network Ablations on two samples of NTU-RGB+D Dataset \cite{shahroudy2016ntu}, showing the comparison between View Dependent, Global Representation and Full Model at $56 \times 56$ resolution for single input view setup.
% %   with  $v_{i} $ $\xrightarrow{}$ $v_j$  setup.
%   }
% %   %%%%%{-5pt}
% \label{fig:network_ablations}
% % \label{fig:onecol}
% \end{figure*}

% \clearpage
\subsection{NTU-RGB+D Dataset \cite{shahroudy2016ntu}}
Refer Section 4.2 in the manuscript for the summarized quantitative analysis on network ablations. Here, we provide the detailed network and loss ablation in terms of quantitative results and qualitative  visualizations on NTU-RGB+D Dataset along with the comparison with existing works.













\begin{figure}
\begin{center}
    \includegraphics[width=0.45\textwidth]{images/ModelAblationCVPR.pdf}
\end{center}
    
% %%%%%{-10pt}
\caption{Qualitative results showing Network Ablations on two samples of NTU-RGB+D Dataset \cite{shahroudy2016ntu}, showing the comparison between View Dependent (tested), Global Representation(tested) and Full Model at $56 \times 56$ resolution for multiple input view setup.
}
\label{fig:NTUNetworkAblationVDGR}
% %%%%%{-10pt}
\end{figure}


\begin{figure}[t]
\begin{center}
% \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
  %\includegraphics[width=0.8\linewidth]{egfigure.eps}
  \includegraphics[width=.45\textwidth]{images/WACVNetworkAblation-Fig1.pdf}
%   %%%%%{-10pt}
\end{center}
  \caption{Qualitative results showing Network Ablations on two samples of NTU-RGB+D Dataset \cite{shahroudy2016ntu}, showing the comparison between View Dependent (trained), Global Representation (trained) and Full Model at $56 \times 56$ resolution for single input view setup.
  }
\label{fig:network_ablations}
\end{figure}



% \begin{table*}[]
%  \small
%   \centering
%   \renewcommand{\tabcolsep}{0.4mm}  
  
%   \caption{\small SSIM, PSNR and FVD   scores for Network Ablations on NTU-RGB+D Dataset \cite{shahroudy2016ntu} using View Dependent (VD) stream, Global Representation (GR) stream and the full model (Full) on $56 \times 56$ resolution. The left panel shows the results for multi-input view setup, whereas the right panel shows single-input view setup results.
% %   Left panel shows results for ($v_{i1} , v_{i2}$) $\xrightarrow{}$ $v_j$ setup; right panel shows results for \textbf{$v_i$ $\xrightarrow{}$ $v_j$} setup. 
% %   \MS{Put on the top of each panels heading: Full Model, etc, captions and text are confusing}.
%   }
% %   %%%%%{10pt}

%   \label{tab:network_ablations_2to1}
%     \begin{tabular}{|c|c|c|c|c|c||c|c|c|c|c|c|c|}
%     \hline
%         % \toprule
%         & & \multicolumn{3}{c|}{\textbf{Multi-Input Setup}} & \textbf{Avg} & \multicolumn{6}{c|}{\textbf{Single Input Setup}} & \textbf{Avg}
%         \\
%         \cline{3-5}  \cline{7-12}
%         % \cline{3-13}
%       \textbf{Network}  &
%         \textbf{Metric} &  \textbf{($v_1 , v_2$) $\xrightarrow{}$ $v_3$} & \textbf{($v_2 , v_3$) $\xrightarrow{}$ $v_1$}  & \textbf{($v_1 , v_3$) $\xrightarrow{}$ $v_2$} & \textbf{Score}  &  \textbf{$v_1$ $\xrightarrow{}$ $v_2$} & \textbf{$v_1$ $\xrightarrow{}$ $v_3$}  & \textbf{$v_2$ $\xrightarrow{}$ $v_1$} & \textbf{$v_2$ $\xrightarrow{}$ $v_3$} & \textbf{$v_3$ $\xrightarrow{}$ $v_1$} & \textbf{$v_3$ $\xrightarrow{}$ $v_2$} & \textbf{Score}
%         \\
%         % \midrule
%         % \midrule
%         \hline
%         \hline
        
%         & \textbf{SSIM($\uparrow$)}  & 0.548 & 0.579 & 0.563 &0.335& 0.539 & 0.517 & 0.548 &0.547&0.537&0.519&0.534 \\


%      \textbf{VD}\small{(tested)}   & \textbf{PSNR($\uparrow$)}  &16.13 & 16.21 & 16.32 &12.58& 15.86 & 15.62 & 15.59 &15.59&15.63&15.747&15.67\\


%       & \textbf{FVD($\downarrow$)}  &16.84 & 16.57 &16.92 &16.77 & 17.48 & 17.37 & 18.93 &17.11&16.90&17.47&17.18 \\


%         \hline

%       &  \textbf{SSIM($\uparrow$)}  & 0.783 & 0.814 & 0.780 &0.792 & 0.781 & 0.777 & 0.804 &0.774&0.799&0.773 & 0.784 \\
  
%       \textbf{GR}\small{(tested)}   &  \textbf{PSNR($\uparrow$)}  & 19.99 & 20.67 &19.50&20.05 & 19.56 & 19.83 &20.2 &19.67&20.04& 19.23  & 19.755 \\
%      \textbf{}  &  \textbf{FVD($\downarrow$)}  & 13.25& 13.54 &13.57&13.45 & 13.69 & 13.17 & 12.12 &13.78&13.17&13.89&13.33 \\
% \hline
        
        
        
        
       
%         & \textbf{SSIM($\uparrow$)}  & 0.548 & 0.579 & 0.563 &0.563& 0.539 & 0.517 & 0.548 &0.547&0.537&0.519&0.534 \\


%      \textbf{VD}\small{(trained)}   & \textbf{PSNR($\uparrow$)}  &16.13 & 16.21 & 16.32 &16.22& 15.86 & 15.62 & 15.59 &15.59&15.63&15.747&15.67\\


%       & \textbf{FVD($\downarrow$)}  &16.84 & 16.57 &16.92 &16.77 & 17.48 & 17.37 & 16.77 &17.11&16.90&17.47&17.18 \\


%         \hline

%       &  \textbf{SSIM($\uparrow$)}  & 0.783 & 0.814 & 0.780 &0.792 & 0.781 & 0.777 & 0.804 &0.774&0.799&0.773 & 0.784 \\
  
%       \textbf{GR}\small{(trained)}   &  \textbf{PSNR($\uparrow$)}  & 19.99 & 20.67 &19.50&20.05 & 19.56 & 19.83 &20.2 &19.67&20.04& 19.23  & 19.755 \\
%      \textbf{}  &  \textbf{FVD($\downarrow$)}  & 13.25& 13.54 &13.57&13.45 & 13.69 & 13.17 & 12.12 &13.78&13.17&13.89&13.33 \\
% \hline

%         & \textbf{SSIM($\uparrow$)}  & 0.801& 0.834 & 0.805 &\textbf{0.813}& 0.804 & 0.793 & 0.828 &0.783&0.815&0.790&\textbf{0.802} \\
        

%       \textbf{Full}  & \textbf{PSNR($\uparrow$)}  & 20.65& 21.40 & 20.34 &\textbf{20.79}& 20.44 & 20.48 & 20.97 &20.17&20.63&20.02&\textbf{20.45}\\

  
%         & \textbf{FVD($\downarrow$)}  & 12.75& 11.25 & 12.93 &\textbf{12.31} & 11.01 & 11.04 & 11.76 &12.78&11.94&12.28&\textbf{11.80}\\

%      \hline

%     \end{tabular}
% \end{table*}


% \begin{figure}
% \begin{center}
%     \includegraphics[width=0.45\textwidth]{images/ModelAblationCVPR.pdf}
% \end{center}
    
% % %%%%%{-10pt}
% \caption{Qualitative results showing Network Ablations on two samples of NTU-RGB+D Dataset \cite{shahroudy2016ntu}, showing the comparison between View Dependent (tested), Global Representation(tested) and Full Model at $56 \times 56$ resolution for multiple input view setup.
% }
% \label{fig:NTUNetworkAblationVDGR}
% % %%%%%{-10pt}
% \end{figure}
% %%%%%{10pt}
\noindent \textbf{Network Ablations.}
We performed two types of ablations for evaluating the role of the global and view-dependent representations. First, we tested the fully trained network by using only one representation at a time. Figure \ref{fig:NTUNetworkAblationVDGR} shows the testing results with global representation $r_g$ and/or view-dependent representation $r_t$. With global representation $r_g$, the foreground and background are almost formed however view-dependent representation $r_t$ is not meaningful alone. The $r_t$ helps by filling in the view specific finer details and only makes sense along with the global representation. It is visibly obvious that best results are obtained with the dual representation $ r $. The detailed quantitative evaluation for single and multi-input setup is shown in Table \ref{tab:network_ablations_2to1} (Row 1-2).



\begin{table*}[]
 \small
  \centering
  \renewcommand{\tabcolsep}{0.4mm}  
  
  \caption{\small SSIM, PSNR and FVD   scores for Network Ablations on NTU-RGB+D Dataset \cite{shahroudy2016ntu} using View Dependent (VD) stream, Global Representation (GR) stream and the full model (Full) on $56 \times 56$ resolution. The left panel shows the results for multi-input view setup, whereas the right panel shows single-input view setup results.
%   Left panel shows results for ($v_{i1} , v_{i2}$) $\xrightarrow{}$ $v_j$ setup; right panel shows results for \textbf{$v_i$ $\xrightarrow{}$ $v_j$} setup. 
%   \MS{Put on the top of each panels heading: Full Model, etc, captions and text are confusing}.
  }
%   %%%%%{10pt}

  \label{tab:network_ablations_2to1}
    \begin{tabular}{|c|c|c|c|c|c||c|c|c|c|c|c|c|}
    \hline
        % \toprule
        & & \multicolumn{3}{c|}{\textbf{Multi-Input Setup}} & \textbf{Avg} & \multicolumn{6}{c|}{\textbf{Single Input Setup}} & \textbf{Avg}
        \\
        \cline{3-5}  \cline{7-12}
        % \cline{3-13}
       \textbf{Network}  &
        \textbf{Metric} &  \textbf{($v_1 , v_2$) $\xrightarrow{}$ $v_3$} & \textbf{($v_2 , v_3$) $\xrightarrow{}$ $v_1$}  & \textbf{($v_1 , v_3$) $\xrightarrow{}$ $v_2$} & \textbf{Score}  &  \textbf{$v_1$ $\xrightarrow{}$ $v_2$} & \textbf{$v_1$ $\xrightarrow{}$ $v_3$}  & \textbf{$v_2$ $\xrightarrow{}$ $v_1$} & \textbf{$v_2$ $\xrightarrow{}$ $v_3$} & \textbf{$v_3$ $\xrightarrow{}$ $v_1$} & \textbf{$v_3$ $\xrightarrow{}$ $v_2$} & \textbf{Score}
        \\
        % \midrule
        % \midrule
        \hline
        \hline
        
        & \textbf{SSIM($\uparrow$)}  & 0.313 & 0.352 & 0.340 &0.335& 0.323 & 0.327 & 0.329 &0.316&0.315&0.323&0.323 \\


     \textbf{VD}\small{(tested)}   & \textbf{PSNR($\uparrow$)}  &12.67 & 13.20 & 11.88 &12.58& 12.09 & 12.52 & 12.59 &11.92&11.89&12.11&12.18\\


      & \textbf{FVD($\downarrow$)}  &18.20 & 18.48 &18.03 &18.23 & 19.23 & 19.93 & 18.96 &18.92&17.78&17.67&18.74 \\


        \hline

       &  \textbf{SSIM($\uparrow$)}  & 0.634 & 0.647 & 0.637 &0.639 & 0.634 & 0.627 & 0.629 &0.624 & 0.628&0.631 & 0.629 \\
  
       \textbf{GR}\small{(tested)}   &  \textbf{PSNR($\uparrow$)}  & 17.23 & 17.72 &17.40&17.45 & 16.12 & 16.96 &16.66 &17.02 & 16.67& 16.31  & 16.62 \\
       
     \textbf{}  &  \textbf{FVD($\downarrow$)}  & 15.45& 15.82 &15.76 & 15.68 & 15.39 & 15.87 & 16.02 & 16.28 & 16.71 &15.39 & 15.94 \\
\hline
        
        
        
        
       
        & \textbf{SSIM($\uparrow$)}  & 0.548 & 0.579 & 0.563 &0.563& 0.539 & 0.517 & 0.548 &0.547&0.537&0.519&0.534 \\


     \textbf{VD}\small{(trained)}   & \textbf{PSNR($\uparrow$)}  &16.13 & 16.21 & 16.32 &16.22& 15.86 & 15.62 & 15.59 &15.59&15.63&15.747&15.67\\


      & \textbf{FVD($\downarrow$)}  &16.84 & 16.57 &16.92 &16.77 & 17.48 & 17.37 & 16.77 &17.11&16.90&17.47&17.18 \\


        \hline

       &  \textbf{SSIM($\uparrow$)}  & 0.783 & 0.814 & 0.780 &0.792 & 0.781 & 0.777 & 0.804 &0.774&0.799&0.773 & 0.784 \\
  
       \textbf{GR}\small{(trained)}   &  \textbf{PSNR($\uparrow$)}  & 19.99 & 20.67 &19.50&20.05 & 19.56 & 19.83 &20.2 &19.67&20.04& 19.23  & 19.755 \\
     \textbf{}  &  \textbf{FVD($\downarrow$)}  & 13.25& 13.54 &13.57&13.45 & 13.69 & 13.17 & 12.12 &13.78&13.17&13.89&13.33 \\
\hline

        & \textbf{SSIM($\uparrow$)}  & 0.801& 0.834 & 0.805 &\textbf{0.813}& 0.804 & 0.793 & 0.828 &0.783&0.815&0.790&\textbf{0.802} \\
        

      \textbf{Full}  & \textbf{PSNR($\uparrow$)}  & 20.65& 21.40 & 20.34 &\textbf{20.79}& 20.44 & 20.48 & 20.97 &20.17&20.63&20.02&\textbf{20.45}\\

  
        & \textbf{FVD($\downarrow$)}  & 12.75& 11.25 & 12.93 &\textbf{12.31} & 11.01 & 11.04 & 11.76 &12.78&11.94&12.28&\textbf{11.80}\\

     \hline

    \end{tabular}
\end{table*}

\begin{table*}[]
 \small
  \centering
  \renewcommand{\tabcolsep}{0.6mm}  
  
  \caption{\small SSIM and PSNR scores for different combination of losses on NTU Dataset\cite{shahroudy2016ntu}  $56 \times 56$ resolution.  
%   Here \textbf{$v_i$ $\xrightarrow{}$ $v_j$} means input view is  $v_i$, query view is $v_j$.
  $L_2$ is the Reconstruction loss, $L_p$ is the Perceptual loss and $L_{adv}$ is the Adversarial loss. The left panel shows the results for multi-input view setup, whereas the right panel shows single-input view setup results.}
%   %%%%%{5pt}
  \label{tab:loss_ablations}
    \begin{tabular}{|l|lcc|c|c|c|c||l|c|c|c|c|c|c|}
        % \toprule
        \hline
         & \multicolumn{3}{c|} {\textbf{Losses}}  & \multicolumn{3}{c|} {\textbf{Multi-Input Setup}} &{\textbf{Avg}}&\multicolumn{6}{c|} {\textbf{Single-Input Setup}}& {\textbf{Avg}}  \\
        
        \cline{2-7}
        \cline{9-14}

        \textbf{\footnotesize{Metrics}}& \footnotesize{$L_2$}  & \footnotesize{$L_p$}& \footnotesize{$L_{adv}$} &  \textbf{($v_1 , v_2$) $\xrightarrow{}$ $v_3$} & \textbf{($v_2 , v_3$) $\xrightarrow{}$ $v_1$}  & \textbf{($v_1 , v_3$) $\xrightarrow{}$ $v_2$} &\footnotesize{\textbf{Score}} &  \footnotesize{$v_1$ $\xrightarrow{}$ $v_2$} & \footnotesize{$v_1$ $\xrightarrow{}$ $v_3$}  & \footnotesize{$v_2$ $\xrightarrow{}$ $v_1$} & \footnotesize{$v_2$ $\xrightarrow{}$ $v_3$} & \footnotesize{$v_3$ $\xrightarrow{}$ $v_1$} & \footnotesize{$v_3$ $\xrightarrow{}$ $v_2$} & \footnotesize{\textbf{Score}} 
        \\
        % \midrule
        % \midrule
        \hline
        \hline
         & \footnotesize{\checkmark}  &&&  0.699& 0.723 & 0.704 &0.708& {0.689} & 0.704 & 0.653 &0.678&0.651&0.670&0.674 \\

        &     &\footnotesize{\checkmark}&\footnotesize{\checkmark}& 0.737& 0.775 & 0.745 &0.752&0.703 & 0.714 & 0.601 &0.710&0.662&0.662&0.675 \\
  
       \textbf{\footnotesize{SSIM}} & \footnotesize{\checkmark}   &\footnotesize{\checkmark}&& 0.791& 0.833 & 0.796 &0.806&0.773 & 0.774 & 0.778 &0.768&0.766&0.749&0.768 \\
        
        \textbf{\footnotesize{($\uparrow$)}} & \footnotesize{\checkmark}   &&\footnotesize{\checkmark}&0.784 & 0.825 &0.789& 0.799& 0.783 & 0.776 & 0.798 &0.761&0.815&0.787& {0.786} \\
        & \footnotesize{\checkmark}   &\footnotesize{\checkmark}&\footnotesize{\checkmark}& 0.801& 0.834 & 0.805 &\textbf{0.813}&0.804 & 0.793 & 0.828 &0.783&0.815&0.790&\textbf{0.802} \\



        \hline
        & \footnotesize{\checkmark}  &&&17.56& 18.55 & 17.89 &18.00& 17.25 & 18.27 & 16.92 &17.27&16.55&17.01&17.21 \\

        &     &\footnotesize{\checkmark}&\footnotesize{\checkmark}& 18.96& 19.94 & 18.78 &19.22&17.85&   18.464 &15.82&18.39&17.34& 17.34&17.53 \\
  
       \textbf{\footnotesize{PSNR}} & \footnotesize{\checkmark}  &\footnotesize{\checkmark}&&  19.69& 21.63& 20.38 &20.72&19.76 & 20.24 & 19.72 &18.03&19.31&18.93&19.29 \\
        
        \textbf{\footnotesize{($\uparrow$)}}& \footnotesize{\checkmark}   &&\footnotesize{\checkmark}& 20.19& 21.06 & 19.91 &20.38&19.76 & 20.00 & 20.15 &18.58&19.55&18.8&19.47 \\
        
         & \footnotesize{\checkmark}  &\footnotesize{\checkmark}&\footnotesize{\checkmark}&20.65& 21.40 & 20.34 &\textbf{20.79}&20.44 & 20.48 & 20.97 &20.17&20.63&20.02&\textbf{20.45} \\


        \hline

    \end{tabular}
\end{table*}

% ------------ FIGURE 5 START ---------------- %
\begin{figure}[]
% \begin{figure}[htbp]
\begin{center}
   \includegraphics[width=0.99\linewidth]{images/NTU112Comparison.pdf}
%   %%%%%{-10pt}
\end{center}
   \caption{Qualitative results on NTU-RGB+D Dataset\cite{shahroudy2016ntu} showing comparison with VDG \cite{ilyes2018pose}, PG$^2$ \cite{ma2017pose}, ResNet \cite{he2015deep} and viewLSTM \cite{lakhal2019view}. We show two samples and the resolution is $112 \times 112$ with single-view input
%   $v^{i} $ $\xrightarrow{}$ $v^j$ 
  setup.}
\label{fig:ntu112_comparison_full}
% %%%%%{-15pt}
\end{figure}



Secondly, we trained the network with only one representation at a time to investigate the impact of each branch in our architecture. 
To examine the role of View Dependent block, we employ View Dependent block $V_T$, in conjunction with Video Encoder $V_E$, and Video Decoder $V_D$ (i.e. Global Representation block $V_G$ is removed). To examine the role of Global Representation block, we employ Global Representation block $V_G$, in conjunction with Video Encoder $V_E$,  and Video Decoder $V_D$ (i.e. View Dependent block $V_T$ is removed).

The final experiment is performed on the full model $i.e.$ $V_T$ and $V_G$ combined. The qualitative results for network ablations are presented in Figure \ref{fig:network_ablations}. The first row shows the frames from input clip, followed by the synthesized outputs for View Dependent (VD) stream, Global Representation (GR) stream and the full model in rows two, three and four respectively. 
Finally, the ground truth frames are shown in the last row. 
The outputs from the network with View Dependent stream contains visible artifacts in the frames. The network with Global Representation stream shows improvements in visual quality of the output over the network with View Dependent branch only. Finally, the full model is able to add finer details like arm and leg (Figure \ref{fig:network_ablations}, right panel) in the synthesized output. 

Table \ref{tab:network_ablations_2to1} (Row 3-4) shows detailed quantitative results for network ablations for single and multiple input-view settings. The quantitative results are consistent for both single and multiple input-view setups, and for all input and output view combinations. The results show that View Dependent and Global Representation streams learn complementary features that are aggregated by the full model (Table \ref{tab:network_ablations_2to1} Row 5) and generate better results.


% %%%%%{10pt}



\begin{table}[t]
 \small
  \centering
\renewcommand{\tabcolsep}{3mm} 
  \caption{\small SSIM scores comparison with existing frame based methods\cite{ilyes2018pose, ma2017pose} and state-of-the-art video-based method, viewLSTM \cite{lakhal2019view} on \textbf{ NTU-RGB+D dataset at 112 $\times$ 112 resolution} with single-view input setup. 
%   \MS{why onle v2 to v3 and v3 to v2 you are getting improvement? the other you are not doing better. Reviewers will ask the explanation? How about other metrics? Are you doing better than viewLSTM?} 
  The scores for viewLSTM \cite{lakhal2019view} are computed for the videos synthesized using both depth and skeleton priors from the query view.}
%   Our method performs better (average score) than SOTA viewLSTM \cite{lakhal2019view}  {\em without using any query-view priors} 

%   \textcolor{blue}{Do you explain why only v3 to v2 and v2 to v3 you do better?. Also, do you just want to put the average, which looks better?}
%   %%%%%{5pt}
  \label{tab:comparison_with_vLSTM_NTU}
    \begin{tabular}{|c|c|c|c|c|}
        % \toprule
        \hline
      Metric  & \multicolumn{4}{c|}{Methods}
        \\
        \cline{2-5}
         &  {\cite{ilyes2018pose}} & {\cite{ma2017pose}}  & {\cite{lakhal2019view}} & \textbf{Ours} 
        \\
         \hline
         \hline
         \textbf{SSIM($\uparrow$)}&  {0.554} & {0.560}  & {0.783} & \textbf{0.791} 
        \\
        \hline
        % \midrule
        % \midrule
        % \hline
        % \cite{ilyes2018pose}  & 0.503 & 0.543 & 0.584 &0.563&0.611&0.522&0.554 \\
        % \cite{ma2017pose}  & 0.499 & 0.561 & 0.600 &0.557&0.598&0.543&0.560 \\
        
        % \cite{lakhal2019view}  & 0.789 & 0.791 & 0.800 &0.765&0.797&0.756&0.783 \\

        % \textbf{Ours}  & 0.786 & 0.784 & 0.790 &0.796&0.793&0.797&\textbf{0.791} \\

         

    \end{tabular}
\end{table}



\begin{figure}[t]
\begin{center}
% \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
  %\includegraphics[width=0.8\linewidth]{egfigure.eps}
  \includegraphics[width=.42\textwidth]{images/NTU112x112CC.pdf}
\end{center}
  %%%%%{-5pt}
  \caption{Qualitative results on NTU-RGB+D Dataset\cite{shahroudy2016ntu} showing comparison with viewLSTM \cite{lakhal2019view}. We show two samples and the resolution is $112 \times 112$ with single-view input
%   $v^{i} $ $\xrightarrow{}$ $v^j$ 
  setup.}
%   %%%%%{-15pt}
\label{fig:NTU112x112Comparison}
% \label{fig:onecol}
\end{figure}



\noindent \textbf{Comparison with Existing Works.}

In order to compare with the existing novel view prediction methods, 
% and also to demonstrate the application of of our network to single-view input, 
we test our network to synthesize a query view video using a single view video as input.
% As a special case, we tested our network to synthesize target view video from single input view video.
% \MS{Tables 2 and 3 are one input view as well; reviewers may get confused, this should be clarified}. 
We input multiple copies of the same input clip, as explained earlier with CMU Panoptic dataset. The experiment is conducted at 112 $\times$ 112 resolution.
% For training, we follow the same setup with given two randomly selected input views, the third is synthesized by the network. As a special case,  our model can also be tested with single input view by repeatedly feeding one clip for the two inputs. 
We compare with a state-of-the-art video-based method, viewLSTM \cite{lakhal2019view} and two frame-based methods \cite{ilyes2018pose, ma2017pose}. 

The quantitative comparison is shown in Table \ref{tab:comparison_with_vLSTM_NTU}. It can be observed that SSIM with proposed approach is comparable to ViewLSTM \cite{lakhal2019view}, without using any priors from the query view. ViewLSTM \cite{lakhal2019view}, on the other hand, uses multiple priors from the query view, i.e both depth and skeleton information. The frame-based methods \cite{ilyes2018pose, ma2017pose} were reportedly trained to predict smaller view-point changes. When trained on NTU-RGB+D there are larger view point changes and our method predicts better quality videos. Also, these methods are unable to capture the temporal coherency between the synthesized frames. 



\begin{table}[t]
 \small
  \centering
  \renewcommand{\tabcolsep}{2.0mm}  
  \caption{\small  SSIM, PSNR and FVD scores for different combination of losses on NTU-RGB+D Dataset \cite{shahroudy2016ntu} on $56 \times 56$ resolution. 
%   (\textbf{$v^{i1}$, $v^{i2}$)  $\xrightarrow{}$ $v^j$} means $v^{i1}$  is the first input view, $v^{i2}$ is the second input view and  $v^j$ is the query view. 
  }
%   %%%%%{-5pt}
  \label{tab:loss_ablations_2to11}
%   %%%%%{5pt}
    \begin{tabular}{|ccc|c|c|c|}

\hline
  \multicolumn{3}{|c|}{Losses} & \multicolumn{3}{|c|}{Metrics}
        % \hline
\\
\hline
        \footnotesize{$L_2$}  & \footnotesize{$L_p$}& \footnotesize{$L_{adv}$} & \footnotesize{\textbf{SSIM($\uparrow$)}} & \footnotesize{\textbf{PSNR($\uparrow$)}}  & \footnotesize{\textbf{FVD($\downarrow$)}}   \\

        \hline
        \hline
        \footnotesize{\checkmark}  &&& 0.708& 18.00 & 15.42 \\

     & \footnotesize{\checkmark}&\footnotesize{\checkmark}& 0.752& 19.22 & 13.96\\
  
     \footnotesize{\checkmark}   &\footnotesize{\checkmark}&& 0.806& 20.72 & 13.28  \\
        
      \footnotesize{\checkmark}   &&\footnotesize{\checkmark}& 0.799 & 20.38 &13.76 \\
        \footnotesize{\checkmark}   &\footnotesize{\checkmark}&\footnotesize{\checkmark}& \textbf{0.817}& \textbf{20.77} & \textbf{12.31}  \\

        \hline

    \end{tabular}
    %   %%%%%{-10pt}

\end{table}



Figure \ref{fig:NTU112x112Comparison} shows a qualitative comparison between the outputs synthesized by viewLSTM \cite{lakhal2019view} (second row) and our proposed method (third row) on NTU-RGB+D dataset. The samples are shown for three time steps and for two samples. As seen with the SSIM scores, our method produces sharper foreground objects and better background details. 







We provide more qualitative results comparing with our baselines VGD \cite{ilyes2018pose}, PG$^2$ \cite{ma2017pose}, ResNet \cite{he2015deep} and viewLSTM \cite{lakhal2019view} in Figure \ref{fig:ntu112_comparison_full}. As can be seen, the frame-bases baselines VDG and PG$^2$ are not able to produce even the scene structure correctly. ResNet, which is used as a video-based baseline, generates correct scene structure but has visible artifacts present. VDNet produces better results but the video quality is low. Finally, we can observe that the proposed method perfectly generates the background as well as the actor performing the action with better motion as well.

\noindent \textbf{Loss Ablations. }
Figure \ref{fig:loss_ablations} shows the qualitative results obtained by employing different  losses. 
 Using only the reconstruction loss produces very blurry results. Adversarial and perceptual loss combined ($L_p + L_{adv}$) helps in sharpening the frames but does not get the color information and background correctly. Adding perceptual loss with reconstruction loss ($L_2 + L_p$) gets the background information well, but the structures of bodies are not defined. $L_2 + L_{adv}$ also produces sharp results with correct background but lacks in producing correct body structures. Finally, combining $L_2 + L_p + L_{adv}$, we get improved results compared to other losses. 
 
 Table \ref{tab:loss_ablations} shows detailed quantitative results for loss ablations for single input-view settings. The results are consistent for different input and output view combinations. The use of all three losses helps to synthesize query view outputs better than using only one or two loss combinations as validated by the table.




\begin{figure}[]
% \begin{figure}[htbp]
\begin{center}
   \includegraphics[width=0.89\linewidth]{images/LossAblations.pdf}
%   %%%%%{-10pt}
\end{center}
   \caption{\small Qualitative Results for loss ablations on NTU Dataset; We show frames obtained by employing  different losses.
   We obtained the the best visual results  employing  all three losses ($L_2 + L_p + L_{adv}$);  here $L_2$ : Reconstruction Loss,  $L_p$ : Perceptual Loss, $L_{adv}$ : Adversarial Loss.
   }
\label{fig:loss_ablations}
% %%%%%{-15pt}
\end{figure}


% \begin{table*}[]
%  \small
%   \centering
%   \renewcommand{\tabcolsep}{0.6mm}  
  
%   \caption{\small SSIM and PSNR scores for different combination of losses on NTU Dataset\cite{shahroudy2016ntu}  $56 \times 56$ resolution.  
% %   Here \textbf{$v_i$ $\xrightarrow{}$ $v_j$} means input view is  $v_i$, query view is $v_j$.
%   $L_2$ is the Reconstruction loss, $L_p$ is the Perceptual loss and $L_{adv}$ is the Adversarial loss. The left panel shows the results for multi-input view setup, whereas the right panel shows single-input view setup results.}
% %   %%%%%{5pt}
%   \label{tab:loss_ablations}
%     \begin{tabular}{|l|lcc|c|c|c|c||l|c|c|c|c|c|c|}
%         % \toprule
%         \hline
%          & \multicolumn{3}{c|} {\textbf{Losses}}  & \multicolumn{3}{c|} {\textbf{Multi-Input Setup}} &{\textbf{Avg}}&\multicolumn{6}{c|} {\textbf{Single-Input Setup}}& {\textbf{Avg}}  \\
        
%         \cline{2-7}
%         \cline{9-14}

%         \textbf{\footnotesize{Metrics}}& \footnotesize{$L_2$}  & \footnotesize{$L_p$}& \footnotesize{$L_{adv}$} &  \textbf{($v_1 , v_2$) $\xrightarrow{}$ $v_3$} & \textbf{($v_2 , v_3$) $\xrightarrow{}$ $v_1$}  & \textbf{($v_1 , v_3$) $\xrightarrow{}$ $v_2$} &\footnotesize{\textbf{Score}} &  \footnotesize{$v_1$ $\xrightarrow{}$ $v_2$} & \footnotesize{$v_1$ $\xrightarrow{}$ $v_3$}  & \footnotesize{$v_2$ $\xrightarrow{}$ $v_1$} & \footnotesize{$v_2$ $\xrightarrow{}$ $v_3$} & \footnotesize{$v_3$ $\xrightarrow{}$ $v_1$} & \footnotesize{$v_3$ $\xrightarrow{}$ $v_2$} & \footnotesize{\textbf{Score}} 
%         \\
%         % \midrule
%         % \midrule
%         \hline
%         \hline
%          & \footnotesize{\checkmark}  &&&  0.699& 0.723 & 0.704 &0.708& {0.689} & 0.704 & 0.653 &0.678&0.651&0.670&0.674 \\

%         &     &\footnotesize{\checkmark}&\footnotesize{\checkmark}& 0.737& 0.775 & 0.745 &0.752&0.703 & 0.714 & 0.601 &0.710&0.662&0.662&0.675 \\
  
%       \textbf{\footnotesize{SSIM}} & \footnotesize{\checkmark}   &\footnotesize{\checkmark}&& 0.791& 0.833 & 0.796 &0.806&0.773 & 0.774 & 0.778 &0.768&0.766&0.749&0.768 \\
        
%         \textbf{\footnotesize{($\uparrow$)}} & \footnotesize{\checkmark}   &&\footnotesize{\checkmark}&0.784 & 0.825 &0.789& 0.799& 0.783 & 0.776 & 0.798 &0.761&0.815&0.787& {0.786} \\
%         & \footnotesize{\checkmark}   &\footnotesize{\checkmark}&\footnotesize{\checkmark}& 0.801& 0.834 & 0.805 &\textbf{0.813}&0.804 & 0.793 & 0.828 &0.783&0.815&0.790&\textbf{0.802} \\



%         \hline
%         & \footnotesize{\checkmark}  &&&17.56& 18.55 & 17.89 &18.00& 17.25 & 18.27 & 16.92 &17.27&16.55&17.01&17.21 \\

%         &     &\footnotesize{\checkmark}&\footnotesize{\checkmark}& 18.96& 19.94 & 18.78 &19.22&17.85&   18.464 &15.82&18.39&17.34& 17.34&17.53 \\
  
%       \textbf{\footnotesize{PSNR}} & \footnotesize{\checkmark}  &\footnotesize{\checkmark}&&  19.69& 21.63& 20.38 &20.72&19.76 & 20.24 & 19.72 &18.03&19.31&18.93&19.29 \\
        
%         \textbf{\footnotesize{($\uparrow$)}}& \footnotesize{\checkmark}   &&\footnotesize{\checkmark}& 20.19& 21.06 & 19.91 &20.38&19.76 & 20.00 & 20.15 &18.58&19.55&18.8&19.47 \\
        
%          & \footnotesize{\checkmark}  &\footnotesize{\checkmark}&\footnotesize{\checkmark}&20.65& 21.40 & 20.34 &\textbf{20.79}&20.44 & 20.48 & 20.97 &20.17&20.63&20.02&\textbf{20.45} \\


%         \hline

%     \end{tabular}
% \end{table*}
% \bibliographystyle{IEEEbib}
% \bibliography{strings,refs}

% \end{document}

